A Note on the Performance of Algorithms for Solving Linear Diophantine Equations in the Naturals

We implement four algorithms for solving linear Diophantine equations in the naturals: a lexicographic enumeration algorithm, a completion procedure, a graph-based algorithm, and the Slopes algorithm. As already known, the lexicographic enumeration algorithm and the completion procedure are slower than the other two algorithms. We compare in more detail the graph-based algorithm and the Slopes algorithm. In contrast to previous comparisons, our work suggests that they are equally fast on small inputs, but the graph-based algorithm gets much faster as the input grows. We conclude that implementations of AC-unification algorithms should use the graph-based algorithm for maximum efficiency.

==> tableNoEpsFull.tex <==

\begin{figure}
\begin{center}
\begin{tabular}{c@{\hspace{0.5cm}}c@{\hspace{0.5cm}}c@{\hspace{0.5cm}}c@{\hspace{0.5cm}}c@{\hspace{0.5cm}}c@{\hspace{0.5cm}}c@{\hspace{0.5cm}}c@{\hspace{0.5cm}}c@{\hspace{0.5cm}}c@{\hspace{0.5cm}}c}
\hline
& A & 2 & 3 & 5 & 13 & 29 & 39 & 107 & 503 & 1021 \\
N & M \\
\hline
1 & 2 & 5:5  & 4:6  & 4:6  & 1:9  & 5:5  & 4:6  & 1:9  & 0:10  & 0:10 \\
1 & 3 & 2:8  & 6:4  & 4:6  & 0:10  & 1:9  & 2:8  & 1:9  & 0:10  & 0:10 \\
1 & 4 & 2:8  & 6:4  & 3:7  & 3:7  & 2:8  & 3:7  & 1:9  & 0:10  & 0:10 \\
1 & 5 & 5:5  & 2:8  & 2:8  & 3:7  & 1:9  & 1:9  & 0:10  & 0:10  & 0:10 \\
1 & 6 & 6:4  & 1:9  & 2:8  & 1:9  & 1:9  & 2:8  & 0:10  & 0:10  & 0:10 \\
1 & 7 & 2:8  & 4:6  & 1:9  & 1:9  & 0:10  & 0:10  & 0:10  & 0:10  & 0:10 \\
1 & 8 & 3:7  & 2:8  & 2:8  & 4:6  & 0:10  & 0:10  & 0:10  & 0:10  & 0:10 \\
1 & 9 & 3:7  & 3:7  & 1:9  & 2:8  & 0:10  & 0:10  & 0:10  & 0:10  & 0:10 \\
\hline
2 & 2 & 5:5  & 5:5  & 5:5  & 2:8  & 1:9  & 1:9  & 0:10  & 0:10  & 0:10 \\
2 & 3 & 5:5  & 3:7  & 3:7  & 3:7  & 3:7  & 0:10  & 4:6  & 4:6  & 9:1 \\
2 & 4 & 4:6  & 3:7  & 0:10  & 2:8  & 0:10  & 1:9  & 5:5  & 10:0  & 10:0 \\
2 & 5 & 1:9  & 2:8  & 3:7  & 1:9  & 0:10  & 5:5  & 9:1  & 8:2  & 10:0 \\
2 & 6 & 2:8  & 0:10  & 2:8  & 2:8  & 3:7  & 4:6  & 8:2  & 10:0  & 8:2 \\
2 & 7 & 4:6  & 3:7  & 7:3  & 3:7  & 4:6  & 8:2  & 8:2  & 10:0  & 4:6 \\
2 & 8 & 5:5  & 4:6  & 7:3  & 4:6  & 3:7  & 9:1  & 9:1  & 9:1  & 6:4 \\
\hline
3 & 3 & 4:6  & 4:6  & 6:4  & 4:6  & 4:6  & 5:5  & 3:7  & 8:2  & 10:0 \\
3 & 4 & 5:5  & 8:2  & 3:7  & 5:5  & 1:9  & 5:5  & 7:3  & 9:1  & 10:0 \\
3 & 5 & 6:4  & 4:6  & 4:6  & 6:4  & 6:4  & 6:4  & 8:2  & 10:0  & 5:5 \\
3 & 6 & 5:5  & 6:4  & 4:6  & 4:6  & 0:10  & 1:9  & 10:0  & 5:5  & 6:4 \\
\hline
4 & 4 & 3:7  & 7:3  & 3:7  & 5:5  & 2:8  & 5:5  & 8:2  & 7:3  & 7:3 \\
4 & 5 & 5:5  & 7:3  & 4:6  & 3:7  & 2:8  & 1:9  & 8:2  & 7:3  & 5:5 \\

\hline
\end{tabular}
\caption{\label{fig11}Comparison of the Graph and Slopes algorithms.
The Graph algorithm wins in 25 test classes and the slopes algorithm wins in 78.}
\end{center}
\end{figure}


==> tableSumTimeFull.tex <==

\begin{figure}
\begin{center}
\begin{tabular}{c@{\hspace{0.5cm}}c@{\hspace{0.5cm}}c@{\hspace{0.5cm}}c@{\hspace{0.5cm}}c@{\hspace{0.5cm}}c@{\hspace{0.5cm}}c@{\hspace{0.5cm}}c@{\hspace{0.5cm}}c@{\hspace{0.5cm}}c@{\hspace{0.5cm}}c}
\hline
& A & 29 & 39 & 107 & 503 & 1021 \\
N & M \\
\hline
1 & 2 & .0:.0  & .0:.0  & .0:.0  & .0:.0  & .1:.0 \\
1 & 3 & .0:.0  & .0:.0  & .0:.0  & .1:.0  & .1:.0 \\
1 & 4 & .0:.0  & .0:.0  & .1:.0  & .2:.0  & .8:.0 \\
1 & 5 & .0:.0  & .0:.0  & .1:.0  & 2.7:.1  & 5.7:.2 \\
1 & 6 & .0:.0  & .0:.0  & .1:.0  & 9.8:.4  & 27.1:1.0 \\
1 & 7 & .0:.0  & .1:.1  & .7:.1  & 29.7:.5  & 184.4:4.0 \\
1 & 8 & .1:.0  & .1:.0  & 2.0:.2  & 206.0:1.6  & 1596.9:24.4 \\
1 & 9 & .2:.1  & .1:.0  & 7.5:.9  & 798.5:2.8  & 1363.1:308.7 \\
\hline
2 & 2 & .0:.0  & .0:.0  & .0:.0  & .1:.0  & .2:.0 \\
2 & 3 & .0:.0  & .0:.0  & .0:.0  & 4.6:.6  & 10.0:4.0 \\
2 & 4 & .0:.0  & .0:.0  & .2:.2  & 1.5:49.1  & 7.8:310.9 \\
2 & 5 & .0:.0  & .0:.0  & .5:3.2  & 51.5:1191.2  & 99.3:2507.3 \\
2 & 6 & .0:.1  & .2:.2  & 4.3:12.1  & 118.7:3001.0  & 1739.0:3001.0 \\
2 & 7 & .2:.1  & .3:.7  & 6.0:84.0  & 622.1:3001.1  & 2849.7:2428.3 \\
2 & 8 & .6:.5  & 1.0:1.9  & 36.6:905.6  & 2551.7:3001.3  & 3001.3:2712.9 \\
\hline
3 & 3 & .4:.3  & .4:.4  & .8:.8  & 20.8:294.3  & 82.5:2327.9 \\
3 & 4 & .6:.5  & .6:.7  & 2.6:6.2  & 266.5:2227.2  & 1084.1:3001.4 \\
3 & 5 & .5:.5  & .5:.6  & 20.9:74.3  & 1331.5:3001.3  & 2618.1:3001.4 \\
3 & 6 & 56.5:17.5  & 1.7:1.1  & 39.8:275.0  & 2866.9:3001.3  & 3001.3:3001.4 \\
\hline
4 & 4 & .9:.7  & 1.7:2.9  & 36.0:190.5  & 2114.5:2854.4  & 3001.3:3001.4 \\
4 & 5 & 1.8:1.6  & 2.6:2.0  & 177.9:1117.7  & 3001.4:3001.4  & 3001.4:3001.5 \\

\hline
\end{tabular}
\caption{\label{fig44}The total time spent for each algorithm (Graph and Slopes) on each test class. 
We ommited the columns that had the times near zero. The Graph algorithm spent in total 38095.83 seconds and the Slopes algorithm spent in total 55986.14 seconds.}
\end{center}
\end{figure}


==> tableTimeoutsFull.tex <==

\begin{figure}
\begin{center}
\begin{tabular}{c@{\hspace{0.5cm}}c@{\hspace{0.5cm}}c@{\hspace{0.5cm}}c@{\hspace{0.5cm}}c@{\hspace{0.5cm}}c@{\hspace{0.5cm}}c@{\hspace{0.5cm}}c@{\hspace{0.5cm}}c@{\hspace{0.5cm}}c@{\hspace{0.5cm}}c}
\hline
& A & 2 & 3 & 5 & 13 & 29 & 39 & 107 & 503 & 1021 \\
N & M \\
\hline
1 & 2 & 0:0  & 0:0  & 0:0  & 0:0  & 0:0  & 0:0  & 0:0  & 0:0  & 0:0 \\
1 & 3 & 0:0  & 0:0  & 0:0  & 0:0  & 0:0  & 0:0  & 0:0  & 0:0  & 0:0 \\
1 & 4 & 0:0  & 0:0  & 0:0  & 0:0  & 0:0  & 0:0  & 0:0  & 0:0  & 0:0 \\
1 & 5 & 0:0  & 0:0  & 0:0  & 0:0  & 0:0  & 0:0  & 0:0  & 0:0  & 0:0 \\
1 & 6 & 0:0  & 0:0  & 0:0  & 0:0  & 0:0  & 0:0  & 0:0  & 0:0  & 0:0 \\
1 & 7 & 0:0  & 0:0  & 0:0  & 0:0  & 0:0  & 0:0  & 0:0  & 0:0  & 0:0 \\
1 & 8 & 0:0  & 0:0  & 0:0  & 0:0  & 0:0  & 0:0  & 0:0  & 0:0  & 5:0 \\
1 & 9 & 0:0  & 0:0  & 0:0  & 0:0  & 0:0  & 0:0  & 0:0  & 1:0  & 4:1 \\
\hline
2 & 2 & 0:0  & 0:0  & 0:0  & 0:0  & 0:0  & 0:0  & 0:0  & 0:0  & 0:0 \\
2 & 3 & 0:0  & 0:0  & 0:0  & 0:0  & 0:0  & 0:0  & 0:0  & 0:0  & 0:0 \\
2 & 4 & 0:0  & 0:0  & 0:0  & 0:0  & 0:0  & 0:0  & 0:0  & 0:0  & 0:0 \\
2 & 5 & 0:0  & 0:0  & 0:0  & 0:0  & 0:0  & 0:0  & 0:0  & 0:2  & 0:8 \\
2 & 6 & 0:0  & 0:0  & 0:0  & 0:0  & 0:0  & 0:0  & 0:0  & 0:10  & 3:10 \\
2 & 7 & 0:0  & 0:0  & 0:0  & 0:0  & 0:0  & 0:0  & 0:0  & 0:10  & 9:8 \\
2 & 8 & 0:0  & 0:0  & 0:0  & 0:0  & 0:0  & 0:0  & 0:2  & 7:10  & 10:9 \\
\hline
3 & 3 & 0:0  & 0:0  & 0:0  & 0:0  & 0:0  & 0:0  & 0:0  & 0:0  & 0:7 \\
3 & 4 & 0:0  & 0:0  & 0:0  & 0:0  & 0:0  & 0:0  & 0:0  & 0:7  & 1:10 \\
3 & 5 & 0:0  & 0:0  & 0:0  & 0:0  & 0:0  & 0:0  & 0:0  & 0:10  & 8:10 \\
3 & 6 & 0:0  & 0:0  & 0:0  & 0:0  & 0:0  & 0:0  & 0:0  & 9:10  & 10:10 \\
\hline
4 & 4 & 0:0  & 0:0  & 0:0  & 0:0  & 0:0  & 0:0  & 0:0  & 5:9  & 10:10 \\
4 & 5 & 0:0  & 0:0  & 0:0  & 0:0  & 0:0  & 0:0  & 0:2  & 10:10  & 10:10 \\

\hline
\end{tabular}
\caption{\label{fig33}Number of timeouts (10 minutes) for the Graph and Slopes algorithms. 
The Graph algorithm has 102 timeouts and the Slopes algorithm has 175.}
\end{center}
\end{figure}


==> tableWithEpsFull.tex <==

\begin{figure}
\begin{center}
\begin{tabular}{c@{\hspace{0.5cm}}c@{\hspace{0.5cm}}c@{\hspace{0.5cm}}c@{\hspace{0.5cm}}c@{\hspace{0.5cm}}c@{\hspace{0.5cm}}c@{\hspace{0.5cm}}c@{\hspace{0.5cm}}c@{\hspace{0.5cm}}c@{\hspace{0.5cm}}c}
\hline
& A & 2 & 3 & 5 & 13 & 29 & 39 & 107 & 503 & 1021 \\
N & M \\
\hline
1 & 2 & 5:5  & 5:5  & 5:5  & 5:5  & 5:5  & 5:5  & 5:5  & 5:5  & 4:5 \\
1 & 3 & 5:5  & 5:5  & 5:5  & 5:5  & 5:5  & 5:5  & 5:5  & 4:5  & 4:5 \\
1 & 4 & 5:5  & 5:5  & 5:5  & 5:5  & 5:5  & 5:5  & 5:5  & 2:7  & 1:9 \\
1 & 5 & 5:5  & 5:5  & 5:5  & 5:5  & 5:5  & 5:5  & 4:5  & 0:9  & 0:10 \\
1 & 6 & 5:5  & 5:5  & 5:5  & 5:5  & 5:5  & 5:5  & 2:7  & 1:9  & 0:9 \\
1 & 7 & 5:5  & 5:5  & 5:5  & 5:5  & 5:5  & 4:5  & 1:8  & 1:9  & 0:10 \\
1 & 8 & 5:5  & 5:5  & 5:5  & 5:4  & 4:6  & 4:5  & 1:9  & 0:9  & 0:10 \\
1 & 9 & 5:5  & 5:5  & 5:5  & 5:5  & 4:6  & 4:6  & 1:9  & 0:10  & 1:9 \\
\hline
2 & 2 & 5:5  & 5:5  & 5:5  & 5:5  & 5:5  & 5:5  & 5:5  & 4:5  & 2:7 \\
2 & 3 & 5:5  & 5:5  & 5:5  & 5:5  & 5:5  & 5:5  & 5:5  & 6:4  & 9:1 \\
2 & 4 & 5:5  & 5:5  & 5:5  & 5:5  & 5:5  & 5:5  & 6:4  & 10:0  & 10:0 \\
2 & 5 & 5:5  & 5:5  & 5:5  & 5:5  & 5:5  & 5:5  & 9:0  & 8:2  & 10:0 \\
2 & 6 & 5:5  & 5:5  & 5:5  & 5:5  & 5:5  & 4:6  & 8:2  & 10:0  & 8:2 \\
2 & 7 & 5:5  & 5:4  & 5:5  & 5:5  & 4:5  & 8:2  & 8:2  & 10:0  & 5:5 \\
2 & 8 & 5:4  & 4:5  & 6:4  & 4:5  & 4:6  & 6:4  & 9:0  & 7:3  & 5:4 \\
\hline
3 & 3 & 4:5  & 5:5  & 5:5  & 5:4  & 4:5  & 4:6  & 3:6  & 8:2  & 10:0 \\
3 & 4 & 4:5  & 7:3  & 5:5  & 5:5  & 3:7  & 4:5  & 7:3  & 9:1  & 9:0 \\
3 & 5 & 4:5  & 4:6  & 5:5  & 5:5  & 5:5  & 5:4  & 8:1  & 10:0  & 5:4 \\
3 & 6 & 5:4  & 5:5  & 3:6  & 4:6  & 0:9  & 1:9  & 10:0  & 5:5  & 5:4 \\
\hline
4 & 4 & 4:6  & 5:4  & 4:6  & 4:5  & 2:7  & 6:4  & 8:2  & 7:2  & 5:4 \\
4 & 5 & 6:4  & 5:4  & 5:5  & 3:7  & 2:8  & 1:8  & 8:2  & 5:4  & 6:4 \\

\hline
\end{tabular}
\caption{\label{fig22}Comparison of the Graph and Slopes algorithms using an Epsilon of 0.01. The Graph algorithm wins in 22 test classes and the Slopes algorithm wins 18.}
\end{center}
\end{figure}

